Towards Fair Classification against Poisoning Attacks

Fair classification aims to stress the classification models to achieve the equality (treatment or prediction quality) among different sensitive groups. However, fair classification can be under the risk of poisoning attacks that deliberately insert malicious training samples to manipulate the trained classifiers' performance. In this work, we study the poisoning scenario where the attacker can insert a small fraction of samples into training data, with arbitrary sensitive attributes as well as other predictive features. We demonstrate that the fairly trained classifiers can be greatly vulnerable to such poisoning attacks, with much worse accuracy & fairness trade-off, even when we apply some of the most effective defenses (originally proposed to defend traditional classification tasks). As countermeasures to defend fair classification tasks, we propose a general and theoretically guaranteed framework which accommodates traditional defense methods to fair classification against poisoning attacks. Through extensive experiments, the results validate that the proposed defense framework obtains better robustness in terms of accuracy and fairness than representative baseline methods.

==> sections/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA
  \item Did you mention the license of the assets?
    \answerNA
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/unused.tex <==
\textbf{The Auxiliary Classification Model.} Our method share the similar high-level idea as SEVER~\citep{diakonikolas2019sever}, to find data points with abnormal gradients. Specifically, in our method, we first train an \textit{Auxiliary classification model} $f_{aux}: x \rightarrow (y, z)$ which aims to predict the label $y$ and the sensitive attribute $z$ simultaneously. Generally, RFC aims to find abnormal samples which can hurt the $f_{aux}$'s ability to correctly predict the samples from each subgroup $(Y_u , Z_v)$. Here, we use $(u, v)$ to denote the index of each subgroup.

During the procedure of RFC, in the auxiliary classification task, we treat each subgroup $(Y_u, Z_v)$ as an individual class. For example, given a sample $(x,y,z)$, we use the one-hot encoding $s = [\1(y = Y_1, z = Z_1), ..., \1(y = Y_k, z = Z_m)]$ to represent the new label $s$. (Note: $k$ and $m$ are the size of $\mathcal{Y}$ and $\mathcal{Z}$). 
Then, one can construct a linear classifier with a weight matrix $W\in \R^{(km)\times d}$ which makes the prediction by $f_{aux}(x, W) = \argmax_{i\in \mathcal{Y}\times\mathcal{Z}} ( x\cdot W^T)_i$ and minimize the loss function, such as CrossEntropy. Thus, we can define the centered gradient matrix for each row $W^{uv}$ of the $W$. 
\begin{align}\label{eq:q_matrix}
    Q^{u,v} = \left[\frac{\partial l(f_{aux}(x_i, W), s)}{\partial W^{u,v}} - \sum_{j=1}^n \frac{\partial l (f_{aux}(x_j, W), s)}{\partial W^{u,v}} \right]_{i \in (Y_u, Z_v)}
\end{align}
Notably, each $Q^{u,v}$ has the shape $n\times d$, as $n$ is the number of training samples. Each row of $W^{u,v}$ represents the sample $i$'s centered gradients of weight vector $W^{u,v}$. 
